MUSE: Feature Self-Distillation with Mutual Information and Self-Information

We present a novel information-theoretic approach to introduce dependency among features of a deep convolutional neural network (CNN). The core idea of our proposed method, called MUSE, is to combine MUtual information and SElf-information to jointly improve the expressivity of all features extracted from different layers in a CNN. We present two variants of the realization of MUSE -- Additive Information and Multiplicative Information. Importantly, we argue and empirically demonstrate that MUSE, compared to other feature discrepancy functions, is a more functional proxy to introduce dependency and effectively improve the expressivity of all features in the knowledge distillation framework. MUSE achieves superior performance over a variety of popular architectures and feature discrepancy functions for self-distillation and online distillation, and performs competitively with the state-of-the-art methods for offline distillation. MUSE is also demonstrably versatile that enables it to be easily extended to CNN-based models on tasks other than image classification such as object detection.

==> chapters/tables/muse_fig.tex <==
\begin{table}
% \vspace{-1em}
\small
\centering
\setlength{\tabcolsep}{0.5pt}
\begin{tabular}{c} 
\includegraphics[width=0.25\textwidth]{chapters/figures/final_SI_add.pdf} 
\\
 \includegraphics[width=0.25\textwidth]{chapters/figures/final_SI_multi.pdf} 
%  & (c) & (d) 
 \\
\end{tabular}
\vspace{-1em}
\caption{\textbf{(a) and (b) Training curves of SI loss on CIFAR100 EfficientNet-B0.} X-axis: training steps (per 100 iterations), y-axis: loss (always positive, lower means higher SI). \textcolor{s1}{Orange}, \textcolor{s2}{purple}, \textcolor{s3}{magenta} denote the SI loss of \textcolor{s1}{$F_1$}, \textcolor{s2}{$F_2$} and \textcolor{s3}{$F_3$}. The value of each SI loss is comparable as its implementation is same for all. \textbf{(c) Different terms in MUSE.} \textbf{(d) Compact networks by MUSE.}}
% \label{table:discrepancy}
\end{table}
% \vspace{-2em}
